Compelling Evidence for a Harmonic in the Light Curve of the Supermassive Black Hole Binary Candidate PKS J1309+1154

We recently discovered a supermassive black hole binary (SMBHB) candidate, PKS J1309+1154, in the combined 46-yr University of Michigan Radio Astronomy Observatory (UMRAO) plus Owens Valley Radio Observatory (OVRO) blazar monitoring programs at 14.5/15 GHz. The light curve of PKS 1309+1154 exhibits a 17.9 year periodicity. We also reported a hint of a first harmonic with a 9 year periodicity in this object. Further analysis of the PKS J1309+1154 light curve provides compelling evidence that both the fundamental and the harmonic are real, confirming the existence of real periodicities in blazar light curves. This is the first case, to our knowledge, of watertight evidence for a fundamental and a harmonic periodicity in a blazar light curve. It makes PKS J1309+1154 a \textit{strong\/} supermassive black hole binary (SMBHB) candidate, and thus the third such candidate to be revealed through long-term radio monitoring, the other two being PKS J0805--0111 and PKS 2131--021, both discovered through the OVRO 40 m Telescope monitoring program. It is argued that hundreds of SMBHB candidates will be discovered by the Vera Rubin and Simons Observatories. Coherent searches for gravitational waves from a network of SMBHB candidates, starting immediately, are strongly motivated.

==> macros.tex <==
% MACROS.TEX contains generally useful macros, but not those specifically 
%            useful for paper formats.
%
\newcount\figureno  \newcount\tableno
\figureno=0         \tableno=0
%
\newbox\tablebox    \newdimen\tablewidth
%
\newbox\marginbox
\def\strutdepth{\dp\strutbox}
\def\strutheight{\ht\strutbox}
%
\def\smallformat{\hsize=5.5truein\hoffset=0.5truein
    \vsize=8truein\voffset=0.5truein\parskip=1pt}
\def\largeformat{\hsize=6.5truein\hoffset=0.0truein
    \vsize=8.5truein\voffset=0.0truein}
%
\newcount\sectionnumber \newcount\subsectionnumber 
\newcount\subsubsectionnumber
\sectionnumber=0 \subsectionnumber=0 \subsubsectionnumber=0
%
\def\secno{\ifcase\sectionnumber\or
     I\or II\or III\or IV\or V\or VI\or VII\or VIII\or IX\or
     X\or XI\or XII\fi}
\def\subsecno{\ifcase\subsectionnumber\or
     a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\fi}
\def\subsubsecno{\ifcase\subsubsectionnumber\or
     i\or ii\or iii\or iv\or v\or vi\or vii\or viii\or ix\or x\fi}
%
\def\section#1\par{\advance\sectionnumber by 1 \subsectionnumber=0
    \vskip 14pt plus 3pt minus 3pt\goodbreak
    \centerline{{\sc\secno.\ #1}}\nobreak\medskip}
\def\subsection#1\par{\advance\subsectionnumber by 1 \subsubsectionnumber=0
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\it\subsecno\/})\ {\it #1}}\nobreak\medskip}
\def\subsubsection#1\par{\advance\subsubsectionnumber by 1
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\eightrm\subsubsecno)}\ {\it #1}}\nobreak\medskip}
%
\def\today{\ifcase\month\or
    January\or February\or March\or April\or May\or June\or
    July\or August\or September\or October\or November\or December\fi
    \space\number\day, \number\year}
%
\def\sol{\ifmmode _{\mathord\odot}
         \else $_{\mathord\odot}$\fi}
\def\deg{\ifmmode ^{\circ}
         \else $^{\circ}$\fi}
\def\pdeg{\ifmmode $\setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}
          \else \setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}$\fi}
% Tony's definitions
\def\vs6{{\vskip 6pt \noindent}}
\def\vs15{{\vskip 15pt \noindent}}
%
\def\arcs{\ifmmode {^{\scriptscriptstyle\prime\prime}}
          \else $^{\scriptscriptstyle\prime\prime}$\fi}
\def\arcm{\ifmmode {^{\scriptscriptstyle\prime}}
          \else $^{\scriptscriptstyle\prime}$\fi}
\newdimen\sa  \newdimen\sb
\def\parcs{\sa=.07em \sb=.03em
     \ifmmode $\rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa$
     \else \rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa\fi}
\def\parcm{\sa=.08em \sb=.03em
     \ifmmode $\rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb$
     \else \rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb\fi}
%
\def\s#1{{\sc #1}}
\def\et{\hbox{\it et al.}}
\def\ET{{\it ET AL.}}
\def\expo#1{\ifmmode \times 10^{#1}
            \else $\times 10^{#1}$\fi}
\def\page{\vfill\eject}
\def\leaderfil{\leaders\hbox to 5pt{\hss.\hss}\hfil}
%
\def\mo{\ifmmode ^{-1}
        \else $^{-1}$\fi}
\def\sup#1{$^{\rm #1}$}
\def\mag{\sup{m}}
\def\muK{\,$\mu$\hbox{K}}
\def\,{\thinspace}
\def\tc#1{3C\,#1}
\def\dots{\relax\ifmmode \ldots
          \else $\ldots$\fi}
\def\WHzsr{\ifmmode $W\,Hz\mo\,sr\mo$
           \else W\,Hz\mo\,sr\mo \fi}
\def\mKs{\ifmmode $\,mK\,s$^{-1/2} 
         \else \,mK\,s$^{-1/2}$ \fi}
\def\microns{\ifmmode \,\mu$m$
             \else \,$\mu$m\fi}
\def\micron{\microns}

%
\def\gsim{\lower.6ex\hbox{$\buildrel>\over\sim$}}
\def\lsim{\lower.6ex\hbox{$\buildrel<\over\sim$}}
\def\ra[#1 #2 #3.#4]{#1\sup{h}#2\sup{m}#3\sup{s}\llap.#4}
\def\dec[#1 #2 #3.#4]{#1\deg#2\arcm#3\arcs\llap.#4}
\def\deco[#1 #2 #3]{#1\deg#2\arcm#3\arcs}
%
\def\refindent{\hangindent=1em \hangafter=1 \noindent}
\def\ref #1;#2;#3;#4\par{\refindent #1,{\it #2},{\bf #3},#4.\par}
\def\ajref #1;#2;#3;#4\par{\refindent #1. #2 {\bf #3},#4.\par}
\def\vref #1\par{\refindent #1.\par}
\def\cref #1;#2;#3;#4;#5\par{\refindent #1, in{\it #2}, 
                             \hbox{ed.}#3 #4, \hbox{p.} #5.\par} 
\def\bref #1;#2;#3\par{\refindent #1, {\it #2} (#3).\par}
%
%
\def\tabl #1\par{\centerline{TABLE \number\tableno}
                 \vskip 7pt
                 \centerline{#1}\nointerlineskip\noindent}
\def\endtable{\tablewidth=\wd\tablebox 
    $$\hss\copy\tablebox\hss$$
    \vskip-\lastskip\vskip -2pt}
\def\tablenote#1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=\parindent \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotenoindent #1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=0pt \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotes #1\par{
            \iftform \goodbreak\topinsert{
                 \centerline{NOTES TO TABLE \number\tableno}
                 \vskip .3cm\noindent
                 \eightpoint\input #1 }\endinsert
            \else \iftabsopen\relax
                  \else\immediate\openout\tabs=junk1\tabsopentrue\fi
                \vskip .5cm
                \centerline{NOTES TO TABLE \number\tableno} \vskip .5cm
                \immediate\write\tabs{\string\etable\space#1\string\par}
            \fi}
\def\doubleline{\vskip 3pt\hrule \vskip 1.5pt \hrule \vskip 5pt}
%
% macros for marginal stuff
%
\def\marginstuff#1{\setbox\marginbox=\vtop{
    \hsize=60pt\tolerance=10000\hbadness=10000
%    \hsize=70pt\tolerance=10000\hbadness=10000
    \parindent=0pt\eightpoint#1\par}\strut}
\def\setmarginal{\strut\vadjust{\kern-\strutdepth\kern-\ht\marginbox\vtop{%
    \moveleft 70pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%    \moveleft 80pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%
% macro for absolute positioning on a page
%
\newdimen\offset 
\newdimen\unita \newdimen\unitb
\newdimen\mina  \newdimen\minb 
%
\unita=1.0cm \mina=0.0cm
\unitb=1.0in \minb=0.0in
%
%
\def\point #1 #2 #3;{\offset=#1\unitb\advance\offset by \minb%
    \rlap{\lower\offset\hbox{\hglue #2\unitb #3}}}%
%
% macros for memos
%
\font\ssq=cmssq8 at 7pt \font\ssbx=cmssbx10 at 12pt 
\setbox0=\hbox{\ssq ATENDEES \rm\quad}
\newdimen\atndwd \atndwd=\wd0
\def\file{}
\def\memo{\hsize=5.875in \hoffset=0.3125in
    \vsize=9in     \voffset=0in
    \elevenpoint
    \vglue -0.8in
    \line{\ssq\hfil INTEROFFICE MEMORANDUM\hfil \llap{\twelvepoint\bf\file}}
    \vskip 10pt
    \centerline{\hbox to 5.4in{\ssbx C A L I F O R N I A\hskip 12pt
                I N S T I T U T E\hskip 12pt O F\hskip 12pt 
                T E C H N O L O G Y}}
    \vskip 30pt}
\def\to#1{\line{\ssq TO \rm\quad #1\hfil\today}
          \vskip 12pt}
\def\from#1{\line{\ssq FROM \rm\quad C. R. Lawrence#1\hfil
                  \ssq EXTENSION \rm\quad 4976\quad\quad
                  \ssq MAIL CODE \rm\quad 105-24}
            \vskip 12pt}
\def\subject#1{\line{\ssq SUBJECT \rm\quad#1\hfil}
               \vskip 12pt}
\def\attendees#1{\hangindent=\atndwd \hangafter=1 \noindent
                \ssq ATENDEES \rm\quad#1
                \vskip 24pt}
\def\OVRO#1{\def\file{OVRO 5m \rlap{#1-87}}}

